On structural parameterizations of the selective coloring problem

In the Selective Coloring problem, we are given an integer $k$, a graph $G$, and a partition of $V(G)$ into $p$ parts, and the goal is to decide whether or not we can pick exactly one vertex of each part and obtain a $k$-colorable induced subgraph of $G$. This generalization of Vertex Coloring has only recently begun to be studied by Demange et al. [Theoretical Computer Science, 2014], motivated by scheduling problems on distributed systems, with Guo et al. [TAMC, 2020] discussing the first results on the parameterized complexity of the problem. In this work, we study multiple structural parameterizations for Selective Coloring. We begin by revisiting the many hardness results of Demange et al. and show how they may be used to provide intractability proofs for widely used parameters such as pathwidth, distance to co-cluster, and max leaf number. Afterwards, we present fixed-parameter tractability algorithms when parameterizing by distance to cluster, or under the joint parameterizations treewidth and number of parts, and co-treewidth and number of parts. Our main contribution is a proof that, for every fixed $k \geq 1$, Selective Coloring does not admit a polynomial kernel when jointly parameterized by the vertex cover number and the number of parts, which implies that Multicolored Independent Set does not admit a polynomial kernel under the same parameterization.

==> overview.tex <==
\section{Literature overview}\label{sec:overview}

The original $\NPc$ results of Bodlaender and Jansen~\cite{graph_partitioning1}, despite being initially regarded as polynomial reductions for \pname{Bounded Coloring}, are a nice source of parameterized hardness.
To adapt their proofs to show that \pname{Equitable Coloring} parameterized by the number of colors is \WH\ on cographs and \para\NPH\ on bipartite graphs, it suffices to consider the version of \pname{Bin-Packing} where each bin must be completely filled for the first case, while the latter follows immediately since they prove that \pname{Bounded 3-Coloring} is \NPH\ on bipartite graphs; these imply that adding the distance to theses classes in the parameterization yields no additional power whatsoever.
Fellows et al.~\cite{colorful_treewidth} show that \pname{Equitable Coloring} parameterized by treewidth and number of colors is \WH, while an \XP\ algorithm parameterized by treewidth is given for both \pname{Equitable Coloring} and \pname{Bounded Coloring} by Bodlaender and Fomin~\cite{equitable_treewidth}.
In fact, the reduction shown in~\cite{colorful_treewidth} prove that, even when simultaneously parameterized by feedback vertex set, treedepth, and number of colors, \pname{Equitable Coloring} remains \WH.
Gomes et al.~\cite{equitable_dmtcs} show that the problem parameterized by number of colors, maximum degree and treewidth is \WH\ on interval graphs.
However, their intractability statement can be strengthened to number of colors and \textit{bandwidth}, with no changes to the reduction.
In~\cite{cai_split}, Cai proves that \pname{Vertex Coloring} is \WH\ parameterized by distance to split.

We also reviewed results on parameters weaker than distance to clique, since both distance to cluster and co-cluster fall under this category.
For minimum clique cover, we resort to the classic result of Garey and Johnson~\cite{garey_johnson} that \pname{Partition into Triangles} is \NPH.
By definition, a graph $G$ can be partitioned into vertex-disjoint triangles if and only if its complement graph can be equitably $(n/3)$-colored.
The reduction given in~\cite{garey_johnson} is from \pname{Exact Cover by 3-Sets}, and their gadget (which we reproduce in Figure~\ref{fig:triangles}) has the nice property that the complement graph $\overline{G}$ has a trivial clique cover of size nine: it suffices to pick one gadget $i$ and one clique for each $a_i^j$.
Thus, we have that \pname{Equitable Coloring} is \para\NPH\ parameterized by minimum clique cover.
To see that when also parameterizing by the number of colors there is an \FPT\ algorithm, we first look at the parameterization maximum independent set $\alpha$ and number of colors $k$, both of which we assume to be given on the input.
First, if $k\alpha < n$, the instance is trivially negative, so we may assume $k\alpha \geq n$; but, in this case, we can spend exponential time on the number of vertices and still run in \FPT\ time.
Finally, we reduce from \pname{Equitable Coloring} parameterized by the number of colors $k$ to \pname{Equitable Coloring} parameterized by $k$ and minimum dominating set.
If we take the source graph $G$ and add $\frac{n}{k}$ vertices $D = v_i, \dots, v_{\frac{n}{k}}$ with $N(v_i) = V(G)$ for all $v_i \in D$, the set $\{v_1, u\}$, with $u \in V(G)$, is a dominating set of the resulting graph $G'$; moreover, $G$ has an equitable $k$-coloring if and only if $G'$ is equitably $(k+1)$-colorable, thus proving that \pname{Equitable Coloring} parameterized by $k$ and minimum dominating set is \para\NPH.
A summary of the results discussed in this work is displayed in Figure~\ref{fig:diagram}.

\begin{figure}[!htb]
    \centering
    \begin{tikzpicture}[yscale=0.8, xscale=0.7]
         \GraphInit[unit=3,vstyle=Normal]
         \SetVertexNormal[Shape=circle, FillColor=black, MinSize=3pt]
         \tikzset{VertexStyle/.append style = {inner sep = \inners, outer sep = \outers}}
         \SetVertexLabelOut
         \Vertex[x=-4, y =-3, Lpos=270, Math, L={x_i}]{x}
         \Vertex[x=0, y =-3, Lpos=270, Math, L={y_i}]{y}
         \Vertex[x=4, y =-3, Lpos=270, Math, L={z_i}]{z}
         
         \Vertex[x=-5, y=-2, Lpos=225, Math, Ldist=-1pt, L={a_i^1}]{ax}
         \Vertex[x=-3, y=-2, Lpos=315, Math, Ldist=-1pt, L={a_i^2}]{bx}
         \Edges(ax,x,bx,ax)
         
         \Vertex[x=-1, y=-2, Lpos=225, Math, Ldist=-1pt, L={a_i^4}]{ay}
         \Vertex[x=1, y=-2, Lpos=315, Math, Ldist=-1pt, L={a_i^5}]{by}
         \Edges(ay,y,by,ay)
         
         \Vertex[x=3, y=-2, Lpos=225, Math, Ldist=-1pt, L={a_i^7}]{az}
         \Vertex[x=5, y=-2, Lpos=315, Math, Ldist=-1pt, L={a_i^8}]{bz}
         \Edges(az,z,bz,az)
         
         \Vertex[x=-2.5, y=0, Lpos=135, Math, Ldist=-1pt, L={a_i^3}]{a3}
         \Vertex[x=0, y=-1, Lpos=90, Math, Ldist=-1pt, L={a_i^6}]{a6}
         \Vertex[x=2.5, y=0, Lpos=45, Math, Ldist=-1pt, L={a_i^9}]{a9}
         
         \Edges(ax,a3,bx)
         \Edges(ay,a6,by)
         \Edges(az,a9,bz)
         \Edges(a3,a6,a9,a3)
         
    \end{tikzpicture}
        
    \caption{\pname{Exact Cover by 3-Sets} to \pname{Partition into Triangles} gadget of \cite{garey_johnson} representing the set $C_i = \{x_i,y_i,z_i\}$.}
    \label{fig:triangles}
\end{figure}


\begin{figure}[!htb]
    \hspace{-1.2cm}
    \includegraphics[scale=0.5]{figs/diagram_equitable.pdf}
    \caption{Hasse diagram of the parameterizations of \pname{Equitable Coloring} and their complexities.
    A single shaded box indicates that the problem is \FPT, while a shaded rhombus highlights a case that admits a polynomial kernel; two solid boxes represent \WHness\ even if also parameterized by the number of colors; if the inner box is dashed, the problem is \para\NPH; if the outer box is solid and shaded, additionally using the number of colors results in an \FPT\ algorithm; if it is not shaded, it remains \WH. Entries with a * are our main contributions. Ellipses mark open cases.}
    \label{fig:diagram}
\end{figure}
